Synthetic Cross-language Information Retrieval Training Data

A key stumbling block for neural cross-language information retrieval (CLIR) systems has been the paucity of training data. The appearance of the MS MARCO monolingual training set led to significant advances in the state of the art in neural monolingual retrieval. By translating the MS MARCO documents into other languages using machine translation, this resource has been made useful to the CLIR community. Yet such translation suffers from a number of problems. While MS MARCO is a large resource, it is of fixed size; its genre and domain of discourse are fixed; and the translated documents are not written in the language of a native speaker of the language, but rather in translationese. To address these problems, we introduce the JH-POLO CLIR training set creation methodology. The approach begins by selecting a pair of non-English passages. A generative large language model is then used to produce an English query for which the first passage is relevant and the second passage is not relevant. By repeating this process, collections of arbitrary size can be created in the style of MS MARCO but using naturally-occurring documents in any desired genre and domain of discourse. This paper describes the methodology in detail, shows its use in creating new CLIR training sets, and describes experiments using the newly created training data.

==> _SPP_results_table.tex <==
\begin{table}[b]

\caption{Stage 2 fine-tuning using a single passage in the prompt (SPP)
and \jhpolo's two passages, evaluated on the NeuCLIR 2022 Chinese collection.}
    \label{tab:spp-results}
\centering
\begin{tabular}{ll|cc}
\toprule
Model & Triples & nDCG@20 &  R@100 \\
\midrule
\multirow{2}{*}{ColBERT-X}
& SPP     &   0.190 &  0.254 \\
& \jhpolo &   0.211 &  0.265 \\
\midrule
\multirow{2}{*}{DPR-X}
& SPP     &   0.215 &  0.302 \\
& \jhpolo &   0.192 &  0.294 \\
\bottomrule
\end{tabular}
    
\end{table}

==> _pair_vs_single_example.tex <==
\begin{figure*}
\centering
\setlength{\arrayrulewidth}{0mm}
\begin{tabular}{p{\columnwidth}p{\columnwidth}}
\toprule
\textbf{Document A: }
\begin{CJK*}{UTF8}{bsmi}... 生存,但疫情之下不僅客群少,昂貴租金也讓商家撐不下去,乾脆斷尾求生,這波疫後倒店潮恐難以避免。王鴻薇表示,許多商家向她陳情,本來寒暑假生意就少,這次疫情爆發在5月,無疑雪上加霜,等於有4個月的空窗期,且學校都線上教學,很多店家都撐不下去,大學旁宛如死城,等到開學店家幾乎都倒得差不多了。王舉例,像文大地處陽明山,商家根本不可能做外送訂單,政大附近也有許多店家將近2個月都是暫時休息的狀態,台北醫學大學附近居民也驚呼,「學生開學後,大概店家都要換一輪了。」 王鴻薇補充,助理訪問 ... \end{CJK*}
&
\textbf{Document B:}
\begin{CJK*}{UTF8}{bsmi}
西門商圈來客數狂跌9成 王鴻薇:北市應自發振興消費券 新冠疫情衝擊經濟,近日傳出許多店家宣告倒閉的消息,留下來的只能苦撐待變。對此,台北市議員王鴻薇上午舉行記者會指出,疫情衝擊在三月進入高峰,從觀光旅客來看,港澳與韓國來台旅客數與同期下降八成,以日韓觀光客為消費主力的西門商圈出現海嘯式衝擊,台北車站附近商圈來客數狂跌八到九成。王鴻薇強調,台北市政府不應該再拖了應該要推出台北市自 辦振興消費券,否則商家倒光了也不用救了。 台北市議員王鴻薇上午指出,受到疫情衝擊,台北車站附近商圈來客數狂跌八到九成 ... 
\end{CJK*}
\\
\textbf{Translated Document A: }
... survival, but under the epidemic, not only is there a small number of customers, but also the high rents make businesses unable to survive. They simply cut their tails to survive. This wave of store closures after the epidemic may be inevitable. Wang Hongwei said that many businesses have expressed their feelings to her. Originally, there was little business during the winter and summer vacations. The outbreak of the epidemic in May undoubtedly made things worse. It was equivalent to a 4-month window period, and schools were teaching online. Many businesses could not survive. The neighborhood is like a dead city, and almost all the stores are almost collapsed by the time the school starts. Wang gave an example. For example, Wenda University is located in Yangmingshan, and it is impossible for merchants to order food delivery. There are also many shops near National Chengchi University that have been temporarily closed for nearly two months. Residents near Taipei Medical University also exclaimed, "After the students start school, probably The store will have to change one round.” Wang Hongwei added, assistant interview... 
&
\textbf{Translated Document B:}
The number of visitors in the Ximen commercial district plummeted by 90\%. In this regard, Taipei City Councilor Wang Hongwei held a press conference in the morning and pointed out that the impact of the epidemic reached its peak in March. From the perspective of tourists, the number of tourists from Hong Kong, Macau and South Korea dropped by 80\% compared with the same period in the same period. There was a tsunami-like impact in the shopping district, and the number of visitors to the shopping district near Taipei Main Station plummeted by 80 to 90 percent. Wang Hongwei emphasized that the Taipei City Government should not procrastinate any longer and should launch Taipei City's self-managed revitalization consumer coupons, otherwise there is no need to save businesses if they run out of business. Taipei City Councilor Wang Hongwei pointed out in the morning that due to the impact of the epidemic, the number of visitors to the business district near Taipei Main Station plummeted by 80\% to 90\% ... 
\\
\midrule
\begin{tabular}{p{.95\linewidth}}
\textbf{Generated by SSP with only Document A: } \\
- The impact of the coronavirus pandemic on small businesses in Taiwan. \\
- The lack of customers due to the pandemic and expensive rent. \\
- The trend of businesses closing during the pandemic. 
\end{tabular}
& 
\begin{tabular}{p{.95\linewidth}}
\textbf{Generated by \jhpolo with Document A being Relevant:} \\
- The impact of the pandemic on businesses in Taiwan, particularly those located near universities. \\
- The financial consequences for businesses due to the lack of customers during the pandemic. 
\end{tabular}
\\
\bottomrule
\end{tabular}

    
\caption{Example generated queries using \jhpolo and SPP. }
\label{fig:jhpolo-spp-example}
\end{figure*}
